A Collision Cone Approach for Control Barrier Functions

This work presents a unified approach for collision avoidance using Collision-Cone Control Barrier Functions (CBFs) in both ground (UGV) and aerial (UAV) unmanned vehicles. We propose a novel CBF formulation inspired by collision cones, to ensure safety by constraining the relative velocity between the vehicle and the obstacle to always point away from each other. The efficacy of this approach is demonstrated through simulations and hardware implementations on the TurtleBot, Stoch-Jeep, and Crazyflie 2.1 quadrotor robot, showcasing its effectiveness in avoiding collisions with dynamic obstacles in both ground and aerial settings. The real-time controller is developed using CBF Quadratic Programs (CBF-QPs). Comparative analysis with the state-of-the-art CBFs highlights the less conservative nature of the proposed approach. Overall, this research contributes to a novel control formation that can give a guarantee for collision avoidance in unmanned vehicles by modifying the control inputs from existing path-planning controllers.

==> Experimental_Results.tex <==
\par In this section, the experimental results with Bitcraze\textsuperscript{\texttrademark} Crazyflie 2.1 aerial drone are presented to demonstrate the efficacy of the C3BF controller framework. The global position of the drone as well as the obstacle is measured using Qualisys\textsuperscript{\texttrademark} Miqus M2 motion capture system with a tracking frequency of 100 $Hz$. Further, for the drone, the global position from the motion capture system are fused with the onboard IMU data via Extended Kalmann Filter to the get the filtered state.The control commands are generated by an off board computer and transmitted to the drone via a radio link. The communication with the drone is facilitated through the Crazyflie Python library \cite{cfclient}.

==> controller.tex <==








